Themis: Fair and Efficient GPU Cluster Scheduling

Modern distributed machine learning (ML) training workloads benefit significantly from leveraging GPUs. However, significant contention ensues when multiple such workloads are run atop a shared cluster of GPUs. A key question is how to fairly apportion GPUs across workloads. We find that established cluster scheduling disciplines are a poor fit because of ML workloads' unique attributes: ML jobs have long-running tasks that need to be gang-scheduled, and their performance is sensitive to tasks' relative placement. We propose Themis, a new scheduling framework for ML training workloads. It's GPU allocation policy enforces that ML workloads complete in a finish-time fair manner, a new notion we introduce. To capture placement sensitivity and ensure efficiency, Themis uses a two-level scheduling architecture where ML workloads bid on available resources that are offered in an auction run by a central arbiter. Our auction design allocates GPUs to winning bids by trading off efficiency for fairness in the short term but ensuring finish-time fairness in the long term. Our evaluation on a production trace shows that Themis can improve fairness by more than 2.25X and is ~5% to 250% more cluster efficient in comparison to state-of-the-art schedulers.

==> sections/background.tex <==
\section{ML Training Workload Scheduling Requirements}

In \name{}, we design a cluster scheduler for {\em scheduling a ML training workload in a fair manner}. 
This ML training workload consists of several ML Apps. 
Each ML App comprises of a single or a group of ML training jobs.

In this section, we give a background on the peculiarities of ML Apps and the workload.

\subsection{Specialized Scheduling Logic per ML App}
Each ML App its own unique model architecture, training algorithm, training architecture and training hyperparameters.
These choices make ML Apps heterogeneous and makes the scheduling logic dependent on the specific 
choices that the ML App makes on each of these dimensions.

\subsubsection{Model Architecture}
Deep Neural Nets (DNNs) are a common building block in most ML Apps. 
DNNs can be imagined as a stacking of parameterized layers of neurons. 
This leads to an ever-increasing gamut of model architectures, with some popular ones being 
Convolutional Neural Nets (CNNs), Recurrent Neural Nets (RNNs), Graph Neural Nets (GNNs) and so on. 
Training involves learning the parameters of DNNs and the choice of model architecture imposes unique scheduling requirements. 
For example, training Long Short Term Memory (LSTM) Networks - a type of RNN involves 
sequential computations and training can exclusively be done with CPU resources. 
On the other hand, training CNNs benefits from parallelizable matrix operations and imposes strict GPU resource requirements.
Furthermore, recent works~\cite{soapparallel} have looked at developing model architecture dependent custom scheduling logic for deciding placement of the model operations on a given set of resources.

\subsubsection{Training Algorithm}
The training algorithm for learning the right set of parameters for an ML App can be done via several algorithms.
Some examples are Stochastic Gradient Descent (SGD), Evolution Strategies (ES) and so on. 
The choice of algorithm imposes different scheduling requirements. 

SGD algorithm involves backpropagation to compute gradients which is compute-intensive and imposes GPU resource requirements for a large class of model architectures. 
Furthermore, distributed SGD is typically data-parallelized with multiple workers that compute gradients on different mini-batches of data in parallel. 
Each gradient computation step is followed by a communication step where aggregation and synchronization of the individual gradients calculated by all workers takes place. 
This communication step imposes strict network requirements and several works~\cite{tictac, priorityprop, blueconnect} have looked at developing 
custom communication scheduling logic which 
either optimizes the scheduling of parameter updates depending on the choice of model architecture 
or optimizes communication overhead by exploiting the network interconnect technology available.
Additionally, distributed SGD has an asynchronous variant where the communication step is not a barrier and imposes scheduling requirements involving straggler mitigation strategies.

ES does not involve expensive computation of gradients or an expensive communication aggregation and synchronization step. 
It is embarrassingly parallel and scheduling such an algorithm imposes a large CPU resource requirement. 

\subsubsection{Training Architecture}
Training algorithm such as distributed SGD can be architected in several ways. 
Two common architectures are Parameter Server (PS) architecture and all-reduce architecture.
The training architecture choice imposes several scheduling requirements. 

The PS architecture has several PS processes that hold different shards of the model parameters and worker process that synchronize gradients and parameters via the PS processes. 
This imposes custom scheduling requirements involving 
co-location of PS processes with worker processes to the maximum extent possible, 
gang-scheduling of all processes, 
and CPU and GPU resource requirement for PS process and worker process respectively.

All-reduce architecture has several worker processes that typically synchronize via communication-efficient protocols such as ring-reduce. 
This imposes custom scheduling requirements wherein the worker processes ideally should be placed such that 
they have efficient network technology interconnects such as NVLink between them. 

\subsubsection{Training Hyperparameters}
The training algorithm such as SGD has several hyperparameters such as learning rate, learning algorithm, batch size and so on. 
This imposes custom scheduling logic requirements~\cite{hyperband, hyperdrive} involving reclaiming resources from ML training jobs with poorly converging hyperparameter choices and redistributing to promising job candidates.

\subsection{ML App Workload Characteristics}

\subsubsection{Coarse-Grained Scheduling}
Figure X shows the distribution of ML App running times obtained from an enterprise cluster. 
A large percentage of the jobs, $Y\%$, are long running with runtime >$T min$. 
This makes the case for coarse-grained scheduling and a long-term fairness metric. 

\subsubsection{Placement Sensitive and Unpredictable Running Times}
All ML Apps are sensitive to placement and have unpredictable running times as it is hard to predict point of convergence.
We highlight these trends in Figure X.

\subsubsection{High Contention}
ML Apps execute on a shared GPU cluster. 
GPU resources are scarce leading to high contention for GPU resources among the ML Apps as shown in Figure X.

==> sections/design.tex <==
\section{\name{}}
\label{sec:design}

We now describe the main ideas employed by the \name{} scheduler and
present a design overview. The scheduler attempts to simultaneously
achieve fairness while accounting for placement sensitivity, and
efficiency. %

{\bf Fairness metric.} Our scheduler uses a new metric called {\em
  finish-time fairness}. This is defined as:
    $\rho = \frac{T_{SH}}{T_{ID}}$
i.e., the ratio of the shared running time ($T_{SH}$) to the ideal
running time ($T_{ID}$).  The former ($T_{SH}$) is the estimated
running time of the ML app with its current share of GPU resources in
a cluster shared with $N$ other apps.  The latter ($T_{ID}$) is the
running time of the ML app in a dedicated (un-shared) cluster. Ideally
$\rho$ should be close to (and less than) $N$.

Our scheduling policy (Sec.~\ref{sec:policy}) minimizes the
maximum $\rho$ across apps, while attempting to keep them close to
ideal. We show that this policy ensures sharing incentive
(Sec.~\ref{sec:eval}).


{\bf Semi-optimism and auctions.} Given the constraints imposed by
pessimistic and optimistic architectures, we adopt a middleground.
We use {\em semi-optimistic} inter-app scheduler design that {\em
  separates visibility from allocation}. When GPU resources are
available, our scheduler makes them, along with their locations,
visible to a {\em set} of apps, as opposed to making resources visible
to a single app. Crucially, the set of apps to whom available GPUs are
visible are those whose finish-time fairness metrics are the
worst. Each app in this set places bids on subsets of visible GPUs,
reflecting the placement-sensitive improvement in fairness the app
would derive from acquiring a given subset. Our scheduler runs an
auction that picks a ``winning'' app for each disjoint resource
subset. The set of winning apps maximizes an aggregate function of the
improvements derived, where the function prioritizes efficiency.

{\bf Short-term efficiency and long-term fairness.}  Note that
finish-time fairness reflects the {\em long-term effect} of fair
allocation, which is only apparent when an app terminates. Our
scheduler leverages this by enforcing that apps achieve their ideal
finish-time fair metric by the time they {\em finish}.  By doing so,
our approach balances fairness with efficiency and placement
sensitivity. In particular, on finer minutes-long timescales, when
resource auctions occur, our scheduler may trade off fairness
momentarily to allocate GPUs to apps that place well and can help
maximize efficiency. The momentary deviation from fairness is made up
for during future GPU auctions, as we explain in Section~\ref{sec:semiopt}.






















\begin{figure}[t]
    \centering \includegraphics[width=\columnwidth]{figures/themis-overview.pdf}
    \caption{
        \name{} Design. (a) Sequence of events in \name{} - starting with a pool of resources becoming available and ending with resource allocations. 
        (b) Shows a typical bid valuation table an App submits to \arbiter{}. 
        Each row in the table has a subset of the complete resource allocation and the value of $\rho_{new}$ with this additional allocation. 
    }
    \label{fig:overview}
\end{figure}


\subsection{Design Overview}

Figure~\ref{fig:overview} pictorially shows our architecture. The
cross-app scheduler, i.e., \arbiter{}, is where the scheduling logic is
implemented. The top level per-app schedulers are minimally modified
to interact with the cross-app scheduler.


Each GPU in a \name{}-managed cluster has a lease associated with it.
The lease dictates how long an app can assume ownership of the GPU to
run its workload. When a lease expires, the resource is made available for
allocation. \name{}'s \arbiter{} pools available resources periodically
and makes them visible to ML apps. In particular, the following typical steps ensue
(shown in Figure~\ref{fig:overview}):


\squared{1} The \arbiter{} asks all apps for estimates of their current
finish-time fairness metrics.

\squared{2} The \arbiter{} initiates auctions, by offering available
resources only to a fraction $f \in [0,1]$ of ML apps with {\em worst finish-time
  fair metrics}.  To minimize changes in the ML app scheduler to
participate in auctions, \name{} introduces an \agent{} that is
co-located with each ML app scheduler. The \agent{} serves as an
intermediary between the ML app and the \arbiter{}. The knob $f$
enables trading fairness for efficiency.

\squared{3} The offers received by an app's \agent{} are replied with
        {\em bids}.  To enable preparation of bids, \name{} implements
        a narrow API from the ML app scheduler to the \agent{} that
        enables propagation of app-specific information.  In response
        to an offer, each \agent{} prepares a single bid.  This bid
        contains a {\em valuation function} ($\mathcal{V}$) that
        provides, for each resource subset, a ``value'', i.e., the
        \agent{}'s estimate of the finish-time fair metric the app
        will achieve with the allocation of the resource subset.
        $\mathcal{V}$ is calculated based on app-specific information
        such as placement preferences, total work, current allocation
        and max-parallelism of its constituent jobs
        (Section~\ref{interfaces}).

\squared{4} On receiving all the bids, the \arbiter{} picks winning
bids according to a {\em partial allocation} algorithm
(Section~\ref{auction}), and notifies each \agent{} of its winning
allocation. The algorithm incentivizes truth-telling, is
Pareto-efficient, and allocates all GPUs.

\squared{5} The \agent{} propagates the allocation to the ML app
scheduler, which can then decide how to allocate them among
constituent jobs. 




Thus the above steps reflect how our design achieves finish time
fairness and cluster efficiency across ML applications.

In the following few sections, we first describe how the goal of
cluster-efficiency with finish-time fairness can be translated into an
allocation by the \arbiter{}. Following that we describe the necessary
mechanisms to build a semi-optimistic two level scheduler
corresponding to each step outlined above.









==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\noindent\textbf{Favoring Short Apps.} Our scheduling discipline
implicitly prioritizes apps with small values of $T_{ID}$: If such
jobs don't win initial auctions, then their $\rho$s quickly
deteriorate, making them likely to win allocations in future
auctions. By virtue of their small overall work, such apps can then
complete quickly. Note that this does not affect finish time fairness
for apps with large $T_{ID}$. This property is particularly attractive
for exploratory apps, where users want to quickly examine if a
strawman model is worth improving, or for short apps that have just
one job (with chosen optimal hyper-parameters).


\noindent\textbf{Placement constraints.} Some apps may have placement
constraints due to strict GPU memory requirements for large models.
Our auctions naturally account for app placement constraints: the
valuation table entries for bids containing placement
constraint-violating resource allocations would have infinite $\rho$
value because our placement sensitivity metric, $\mathcal{S}$, for such
resource allocations is $0$.


\noindent\textbf{Early-terminating jobs.} Jobs that are not
going to lead to the best configuration are terminated by
hyperparameter tuning frameworks such Hyperband or Hyperdrive. In this
case, the vacated GPUs are reassigned by these app schedulers to other
running jobs, causing the finish time fairness metric for the app to
drop rapidly. The app will then not be chosen in the following
auctions. However, over time, as the app loses its lease on currently
held GPUs, its finish time metric will increase, bringing the app
back into play in auctions.  This again highlights how our long
term fairness metric automatically accommodates the effect of
early-terminating jobs.

\noindent\textbf{Scheduling after failures.} \name{} may pack apps into
GPUs that share a failure domain. For example, if we allocate all 8
GPUs for a job on a single machine, then a machine failure would mean
the job loses all its resources, stalls in its progress, and has to be
rescheduled immediately to start making progress again.  This could
trigger GPU reallocation {\em away} from other apps currently running on other
machines {\em toward} the rescheduled app. We leave a systematic study of the
effect of failures on scheduling for future work.


==> sections/evaluation.tex <==
\section{Evaluation}
\label{sec:eval}

We evaluate \name{} under a variety of different scenarios through
both testbed driven experiments on a 50 GPU cluster as well through
event-driven simulations.  Since none of the state-of-the-art schemes
are open-source, we benchmark \name{} against them by emulating their
behavior to fit into an auction-based fair market scheme as described
below:


\noindent{\bf Gandiva}\cite{gandiva} is an ML cluster scheduler that aims to 
  improve cluster utilization by introspectively profiling ML app execution, and 
  migrating jobs based on the placement preferences inferred for that job.
  We model Gandiva by having all apps report the placement score for the resources offered, and
    running the same greedy placement algorithm at the end of each lease to
    maximize the placement scores for all apps. 
  We do not model time-slicing of GPUs across jobs since both \name{} and Gandiva would benefit the same amount from it.

  \noindent{\bf Tiresias}~\cite{tiresias} also targets ML workloads but aims to improve average job
    completion time (JCT) using priority-based placements. We model Tiresias using bids by having all apps report 
  their total GPU service. The \arbiter{} assigns resources to apps that have the least GPU service. 
  This model represents a version of Least Acquired Service (LAS) used by Tiresias.

  \noindent{\bf SLAQ}~\cite{slaq} proposes a quality driven scheduling framework that focuses on
    improving aggregate model quality across all jobs. We model SLAQ using bids by having all apps report 
  their decrease in loss value given the resource allocation. 
  The \arbiter{} assigns resources to apps so as to maximize the 
  aggregate decrease in loss with the resource assignment.



\begin{figure*}[t!]
	\centering
	\subfloat[][Variation of Fairness with $f$]{%
		\includegraphics[width=0.30\textwidth]{figures/fairness-knob-fairness.pdf}
		\label{fig:sensitivity_fairness_knob_fairness}
	}
	\subfloat[][Variation of GPU Time with $f$]{%
		\includegraphics[width=0.30\textwidth]{figures/gpu_time_fairness_knob.pdf}%
		\label{fig:sensitivity_fairness_knob_gpu}
	}
	\subfloat[][Variation of Fairness with Lease Time]{%
		\includegraphics[width=0.30\textwidth ,height=3.2cm]{figures/sensitivity-lease-fairness.pdf}%
		\label{fig:sens_lease}
	}
	\caption{ \footnotesize Sensitivity analysis on Fairness Knob $f$ and Lease Time}
\end{figure*}

Our evaluation reveals the below key highlights:
\begin{itemize}
  \item \name{} enables a trade-off between finish-time fairness in the long-term and placement efficiency in the short-term.  
  This is dependent on the choice of fairness knob $f$ and lease time. Sensitivity analysis (Figure~\ref{fig:sensitivity_fairness_knob_fairness}-~\ref{fig:sens_lease}) 
  shows $f \in [0.6,0.8]$ and a lease duration of $20$ min enables significant gains in placement efficiency without sacrificing finish-time fairness. 

  \item \name{} is better than other schemes on finish-time fairness and offers better tail-app completion times, while imposing modest overhead 
  (Figure~\ref{fig:overall_fairness_comparison}-~\ref{fig:job_profile}). 

  \item \name{}'s benefits compared to other schemes improve with increasing fraction of placement sensitive apps and increasing contention in the cluster and 
  these improvements hold even with inaccuracies in finish-time fair metric predictions (Figure~\ref{fig:network_compute}-~\ref{error_impact}). 

\end{itemize}

\subsection{Experimental Setup and Metrics}\label{subsec:setup}

\noindent
{\bf Simulator: } We developed an event-based simulator to evaluate
\name{} at large scale using real traces from a production setting at
a large internet company. We use the traces to obtain a distribution
of the number of hyperparameter exploration jobs per ML
app. The number of tasks per application vary from 1 to 98 with the median as 23. Most tasks within the application require 4 GPUs, but a few of them require just 2 GPUs. Most tasks within an app have short running times (median ~59 minutes), but there are a few long running tasks (median ~123 minutes). We proportionally scale down these times for purpose of our experiments. Our workload consists of a mixture of placement insensitive
(e.g., the ResNet family of models) and placement sensitive (e.g., the
VGG family) applications(60:40 ratio). Since the trace
did not permit actually observing the fidelity (good/promising/bad) of
hyperparameter explorations, for our simulations we assume
clairvoyance of the number of iterations run by each hyperparameter
exploration job. Unless stated otherwise, we evaluate on a
heterogeneously constructed 256 GPU cluster, which has a mixture of 4
GPU, 2 GPU, and 1 GPU machines spread across multiple racks. We model
the inter-arrival times of ML training apps using a Poisson
distribution with a mean inter-arrival time of 20 minutes. We adjust
the contention for GPUs on the cluster by modifying the inter-arrival
time.

\noindent{\bf Testbed Setup: } We run our testbed driven experiments
on Microsoft Azure. Our testbed consists of a cluster of 50 GPUs
spread across 20 instances. We use NC-series and NV-series instances
that have 1/2/4 GPUs in each instance. The GPUs we use include NVIDIA
Tesla K80 and NVIDIA Tesla M60. %

\noindent
{\bf Metrics: } We use a variety of metrics to evaluate \name{}.
\begin{itemize}
	\item {\bf Max Fairness: } The \emph{Max Fairness} metric captures the worst \emph{finish time
    fairness} across apps. Lower values of max fairness indicate a fairer allocation.
	\item {\bf Jain's Fairness: } We use \emph{Jain's Fairness} to measure the variance of
    $\rho=\frac{T_{s}}{T_{i}}$ values across apps. %
    Jain's Fairness close to 1 indicates lower variance in $\rho$ and is better.
    
	\item {\bf Placement Score: } We define a placement score for
          each job in an app depending on the locality of GPUs
          assigned to it. We use a 4-level scoring scheme ranging from
          slot locality, where all GPUs are connected by NVLink,
          machine locality where GPUs are in same machine connected
          over PCIe, rack locality where GPUs are in the same rack,
          and no locality to indicate allocations that cross
          racks. Each successive level has a decrease in network
          bandwidth and would lead to a slowdown (i.e., placement
          sensitivity $\mathcal{S}$) based on application
          properties. A score of 1.0 indicates GPUs are tightly packed
          while lower scores imply GPUs that are spread out.

    
  \item {\bf GPU Time: } We use \emph{GPU Time} as a measure of how efficiently the cluster is
    utilized. For each job across all apps $J_i$, we measure the amount of time it runs on the GPU as $G_{J_i}$ and
    compute total GPU time as $G = \sum_{i=1}^{i=N}{G_{J_i}}$. For two scheduling regimes $S_1$ and
    $S_2$ that have GPU times $G_1$ and $G_2$,  $S_1$ utilizes the cluster more efficiently than
    $S_2$ if $G_1 < G_2$.
\end{itemize}

\subsection{Sensitivity Analysis}\label{subsec:sensitivity_analysis}
In this section, we use simulations of a heterogeneous $256$-GPU
cluster to evaluate the sensitivity of \emph{fairness knob} $f$ and
the lease time to the two metrics that \name{} balances:
\emph{finish-time fairness} and \emph{cluster utilization}.






Figure~\ref{fig:sensitivity_fairness_knob_fairness} shows the impact on \emph{finish-time fairness} as we
vary the fairness knob $f$ which trades off fairness for efficiency. As expected (Section~\ref{sec:semiopt}),  max fairness decreases with an increase in
$f$. 
We also note that the gap between the minimum and
maximum fairness values for a given value of $f$ reduces as $f$ increases. From the plot we also see
that the median finish time fairness increases slightly with $f$ and this is because as discussed in
Section~\ref{sec:policy} the objective for \name{} is to minimize the maximum finish time fairness, and this could come at the expense of median-fairness apps. 
Finally, the figure also shows that
there are diminishing returns and the reduction in maximum finish-time fairness is negligible as we
go from $f=0.8$ to $f=1.0$.


Figure~\ref{fig:sensitivity_fairness_knob_gpu} shows the impact on GPU
time versus $f$. At higher values of $f$, we observe
a higher GPU time implying that the cluster is being used less
efficiently. This is because the visibility of how many apps can bid
for an offer reduces as we increase $f$ leading to fewer opportunities
for the \arbiter{} to pack jobs efficiently. To balance the two , we
choose $f$ as $0.8$ in the rest of our experiments, since we would like
to have better fairness guarantees in multi-tenant settings.




 
Figure~\ref{fig:sens_lease} captures the variation of maximum
\emph{finish-time fairness} as the lease time varies. We observe that
smaller lease times lead to better fairness. This can be attributed to
two factors: (i) decisions on resource allocations across apps at a
finer granularity helps in making more optimal allocations. (ii)
having a shorter lease means that shorter apps do not have long wait
times when they arrive.  A shorter lease time however adds more
overheads since applications would have to be checkpointed and swapped
out more often, and many more auctions must be run. Based on this
observation, we choose a lease time of $20$ minutes for the rest of our
experiments.


\input{sections/evaluation_part2}


==> sections/evaluation_part2.tex <==
\subsection{Macrobenchmarks} \label{subsec:macrobenchmarks}

\begin{figure}
	\centering
	\subfloat[Comparison of Max. Fairness]{\includegraphics[width=0.5\columnwidth]{figures/max_fairness_comparison.pdf}} 
	\subfloat[Comparison of Jain's Index]{\includegraphics[width=0.5\columnwidth]{figures/jf_comparison.pdf}} 
	\caption{\label{fig:overall_fairness_comparison}
		\footnotesize
		Comparison of Finish Time Fairness across different scheduling schemes
	}
\end{figure}

We evaluate \name{} against 
Gandiva, SLAQ, and Tiresias on a cluster of 50 GPUs\footnote{we scaled down the job durations by a factor of 5 and retain the same inter-arrival distribution for our testbed experiments}. 
Figure \ref{fig:overall_fairness_comparison}(a) shows the maximum finish-time fair metric 
for all apps. 
\name{} outperforms all other schedulers. 
In our experiments, the workload resulted in a peak contention of $4.76X$ 
times the number of available GPUs. 
An ideal scheduler would be able to achieve a maximum finish-time fairness of $4.76$. 
\name{} is $\mytilde 7\%$ away from this ideal value. 
In contrast, Gandiva, SLAQ, and Tiresias are $\mytilde 68\%$, $\mytilde 2155\%$, and $\mytilde 1874\%$ away from the ideal, respectively. 
This is expected as Gandiva and SLAQ do not guarantee fairness. 
Tiresias's inefficacy arises from its focus on simple \emph{resource fairness} which ignores placement sensitivity. 

Figure \ref{fig:overall_fairness_comparison}(b) plots Jain's fairness metric across apps. 
Tiresias comes closest and is $\mytilde 5\%$ worse-off than \name{}. 
SLAQ and Gandiva are poorer on fairness as SLAQ demotes old, slowly-converging jobs whereas Gandiva greedily packs with no fairness guarantee. 

\begin{figure}
	\begin{minipage}[t]{0.46\columnwidth}
		\includegraphics[width=\columnwidth]{figures/jct_cdf.pdf}
		\caption{Comparison of App Completion Times across schemes}
		\label{fig:jct_v_others}
	\end{minipage}
	\hspace{0.1cm}
	\begin{minipage}[t]{0.46\columnwidth}
		\includegraphics[width=\columnwidth]{figures/placement_cdf.pdf}
		\caption{CDF of Placement Score}
		\label{fig:placement_benefit}
	\end{minipage}%
\end{figure}

Figure \ref{fig:jct_v_others} shows the job completion times (JCTs) across scheduling schemes. 
\name{} is $\mytilde 4.6\%$, $\mytilde 55.5\%$, and $\mytilde 24.4\%$ better than Gandiva, SLAQ, and Tiresias respectively on average app completion time. 
\name{} is better for two reasons: 
(i) \name{} has visibility into the shared running times of apps over time, and with its long-term focus, makes more frequent allocations to shorter apps than longer ones. 
(ii) \name{} has visibility into different ML apps' placement-sensitivity and packs resources tightly only for the apps that require it. 

\subsubsection{Sources of Improvement} \label{subsubsec:sources_improvement}

\begin{figure}[t]
	\centering \includegraphics[width=0.7\columnwidth]{figures/job_profile.pdf}
	\caption{Timeline of GPU allocations}
	\label{fig:job_profile}
\end{figure}

This section analyzes the reasons \name{} is better. 
Figure \ref{fig:placement_benefit} shows the distribution of placement scores. 
\name{} outperforms other scheduling schemes with Gandiva coming closest. 
Gandiva is not as good as it greedily optimizes for better placement during introspection which does not lead to a good global placement.
Tiresias and SLAQ are much worse as they are placement unaware.

Figure \ref{fig:job_profile} shows a simplified timeline of GPU allocations for $2$ ML apps from our trace. 
For simplicity, we hand-pick two ML apps each having $1$ task. 
The apps vary 3X in their running times and have equal placement sensitivity. 
Both apps arrive at $t=40$. 
The shorter app gets a larger GPU allocation as $\rho$ values are unbounded/large with no allocations and we break ties in favor of shorter apps.
At $t=60$, new apps arrive and the existing apps' leases expire, and our scheme favors allocation to the new app whose $\rho$ is large.
At $t=80$, the shorter app gets GPUs and runs to completion. 
Finally, at $t=120$, the longer app with lesser work remaining continually gets resources and runs to completion. 
This shows \name{} preferentially completes apps with small $T_{ID}$,
but at the same time it does not starve those with high $T_{ID}$.


\subsubsection{System Overheads}


We now evaluate system overheads in \name{}.

From our profiling of the experiments above, we find that each
\agent{} spend ~29 (334) milliseconds to compute bids at the median
(95-\%). The 95 percentile is high because enumeration of possible
bids needs to traverse a larger search space when the number of
resources up for auction is high.

The \arbiter{} uses Gurobi ~\cite{gurobi} to compute partial
allocation of resources to apps based on bids. This computation takes
~354 (1398) milliseconds at the median (95-\%). The high tail is once
again observed when both the number of offered resources and the
number of apps bidding are high. However, the time is small
relative to lease time.

The network
overhead for communication between the \arbiter{} and individual apps
is negligible since we simply leverage the existing mechanisms used by
Apache YARN.

Upon receiving new resource allocations, the \agent{} changes
(adds/removes) the number of GPU containers available to its app. Our
measurements indicate that this change takes about 35-50
seconds. Prior to relinquishing control over its
resources, each application must checkpoint its set of parameters. We
find that that this is model dependent but takes about 5-10 seconds on
an average and is driven largely by the overhead of checkpointing to
HDFS.



\subsection{Microbenchmarks} \label{subsec:microbenchmarks}

This section evaluates the impact of specific characteristics of ML training workloads on 
\emph{finish-time fairness} and \emph{cluster efficiency}. 
Specifically, we evaluate the impact of placement sensitivity and contention for cluster.

\subsubsection{Effect of Placement Sensitivity}

\begin{figure}
	\centering
	\subfloat[Effect on Max. Fairness]{\includegraphics[width=0.5\columnwidth]{figures/max_fairness_deterioration.pdf}} 
	\subfloat[Effect on GPU time]{\includegraphics[width=0.5\columnwidth]{figures/gpu_time_comparison.pdf}} 
	\caption{\label{fig:network_compute}
		\footnotesize
		Impact of placement sensitivity for varying compute-network job distributions
	}
\end{figure}
This experiment analyzes the effect on finish-time fairness and 
cluster efficiency as the fraction of network-intensive apps in 
our workload increases. 


Figure \ref{fig:network_compute}(a) shows the 
factor of improvement in \emph{max fairness} for 
\name{} over Tiresias. 
With only compute-intensive apps, \name{} is only $\mytilde 1.05X$ 
better than Tiresias. 
As the percentage of network-intensive apps increases, 
\name{} performs $\mytilde 2.1x$ better than Tiresias. 
This stems from the fact that placement awareness becomes 
more important when the workload consists of more 
network-intensive ML apps. 

Figure \ref{fig:network_compute}(b) shows the variation in 
\emph{GPU Time} across schemes as we vary the fraction of network-intensive
apps. 
With only compute-intensive apps, all scheduling schemes utilize the cluster with
roughly the same level of efficiency. 
As the percentage of network intensive apps increases, \name{}
utilizes the cluster more efficiently than others. 



\subsubsection{Effect of Contention} \label{subsubsec:contention}

\begin{figure}
	\begin{minipage}[t]{0.48\columnwidth}
		\includegraphics[width=\columnwidth]{figures/fairness_comparison.pdf}
		\caption{Effect of contention on our scheme.}
		\label{contention_effect}
	\end{minipage}
	\hspace{0.1cm}
	\begin{minipage}[t]{0.48\columnwidth}
		\includegraphics[width=\columnwidth]{figures/error_impact.pdf}
		\caption{Impact of error in bid valuations on max fairness}
		\label{error_impact}
	\end{minipage}%
\end{figure}
This experiment analyzes the effect of contention on finish-time fairness. 
Contention is increased by decreasing the inter-arrival times between apps. 

Figure~\ref{contention_effect} shows that the Jain's fairness index worsens more rapidly in Tiresias than \name{}. 
Actual ML training workloads consist of a mixture of medium- to long-sized apps (Section \ref{sec:motivation}). 
\name{} is better than the least attained service mechanism in Tiresias. In addition to being placement-insensitive, because Tiresias prioritizes short and long apps 
equally, it can lead to worse finish-time fairness for short apps.
\name{} with its long-term focus does better on finish-time fairness for both short and long apps. 

\subsubsection{Impact of Error on $\rho$}
This experiment varies the error in bid values in all valuation tables. 
The percentage error is sampled at random from [-$\theta$, $\theta$] range. 
Apps can make errors (not willingly) in computing a new estimate of $\rho$ 
due to error in estimation of work ($\mathcal{W}$) or placement-sensitivity ($\mathcal{S}$). 

Figure \ref{error_impact} shows the changes in max finish-time
fairness as $\theta$ changes.  Note this max finish-time fairness is computed
on accurate $T_{SH}$ and $T_{I}$ values.  Even with $\theta = 0.2$ the
change in max finish-time fairness is not significant.




==> sections/motivation.tex <==
\section{Motivation} \label{sec:motivation}

\name{} is a fair cluster scheduler for ML applications.  We propose a
     {\em long term allocation mechanism} rooted in a new {\em
       finish-time fairness} metric. To realize this, we present a
     novel {\em semi-optimistic} based scheduling architecture which
     uses {\em auctions} as an abstraction.

In this section, we first motivate the need for a new mechanism and
metric by highlighting the drawbacks of existing fair schemes in
supporting the unique features of ML workloads.  We then motivate the
need for a new scheduling architecture by highlighting the drawbacks
of existing schedulers.

\subsection{Definitions}
We define an ML app, or an app for simplicity, as a collection of one
or more ML model {\em training} jobs. Each app corresponds to a user training a
machine learning model for a high-level goal, such as speech recognition or 
object detection. Users train these models knowing the appropriate hyperparameters 
(in which case there is just a single job in the app), 
or they train a closely related set of models ($n$ jobs) that explore hyper-parameters 
such as learning rate, momentum etc.~\cite{hyperdrive,hyperband} 
to identify and train the best target model for the activity at hand.

Each job's constituent work is performed by a number of parallel
\emph{tasks}.  At any given time, all of a job's tasks collectively
process a {\em minibatch} of training data; we assume that the size of
the batch is fixed for the duration of a job. Each task typically
processes a subset of the batch, and, starting from an initial version
of the model, executes multiple iterations of the underlying learning
algorithm to improve the model. We assume all jobs use the
popular synchronous SGD~\cite{google-sync-async}.

We consider the finish time of an app to be when the best model and
relevant hyper-parameters have been identified. Along the course of
identifying such a model, the app may decide to terminate some of its
constituent jobs early~\cite{hyperdrive,hyperopt}; such jobs may be
exploring hyper-parameters that are clearly sub-optimal (the jobs'
model accuracy improvement over iterations is significantly poorer
than other jobs in the same app). For apps that contain a single job,
finish time is the time taken to train this model to a target
accuracy.

\noindent\textbf{Goals.} We seek to design a scheduler for fair and
efficient allocation of cluster GPU resources across such apps.

GPUs are expensive to use and power-hungry. Thus, from a given app's
perspective, a primary attribute of fair resource allocation is that
the performance of the app, i.e., its finish time, from sharing a
cluster $C$ with $N$ other jobs is no worse that $N$ times that when
using $C$ all to itself. If the app's performance is worse, then the
app is better off running in isolation with a $1/N$-sized cluster. We
refer to this as the {\em sharing incentive}.

From the overall cluster's perspective, the available GPU resources
should be used as {\em efficiently} as possible, i.e., overall
GPU-time for a given workload of apps should be small. 






\subsection{Why a new scheduling discipline?}



\begin{figure}
	\begin{minipage}[t]{0.38\columnwidth}
		\includegraphics[width=\columnwidth]{figures/job_duration_cdf.pdf}
		\caption{Distribution of task durations for ML training jobs from an enterprise cluster}
		\label{job-duration}
	\end{minipage}
	\hspace{0.1cm}
	\begin{minipage}[t]{0.5\columnwidth}
		\includegraphics[width=\columnwidth]{figures/placement.pdf}
		\caption{Effect of GPU resource allocation configuration on job throughput for different models.}
		\label{fig:placement}
	\end{minipage}%
\end{figure}






Existing fair allocation schemes, e.g., DRF~\cite{drf}, provide
instantaneous resource fairness.  At any instant that resources become
available, a task from an app with least ``dominant resource share''
is offered resources. These schemes impose two limitations
that violate sharing incentive for ML apps.

\noindent{\bf 1. Short vs long tasks.} Instantaneous resource fairness
assumes that apps have tasks with infinitesimal durations.
For big-data analytics, this is not a limiting assumption and still
approximates resource fairness as tasks are typically
short-lived~\cite{sparrow}, and frequent task completions serve as
opportunities to redistribute resources.  For the case of ML apps,
however, this is a severely limiting assumption as task durations are
typically longer as highlighted in Figure~\ref{job-duration}, and GPU
clusters are heavily contented~\cite{philly-trace-analysis}.  Running
ML tasks to completion could lead to newly arriving jobs waiting
inordinately long for resources and thus lead to violation of the
sharing incentive.




\noindent{\bf 2. Placement sensitivity.}  Placement plays a key role
in rendering existing instantaneous fairness schemes fundamentally
ineffective. ML apps's finish-times are highly sensitive to the
relative placement of their tasks.  Moreover, different ML models have
different placement preferences.  For example, as shown in
Figure~\ref{fig:placement} VGG16 has a strict machine-local task
placement preference while Resnet50 has no such placement preference.
Existing instantaneous resource-fair allocation schemes~\cite{drf} do
not offer apps the ability to express preferences over resources'
relative placement.\footnote{DRF allows jobs to express task demands
  as a vector along resource dimensions, but to model placement of ML
  jobs we need to encode affinity across multiple tasks' demands.}
This mismatch can lead to violation of sharing incentive as a
seemingly resource fair allocation can be very sub-optimal in terms of
placement and lead to higher finish-time for an app. Waiting for
optimally placed resource~\cite{delay} is not an option as ML apps
have long task durations and this will aggravate waiting time for
tasks.

{\bf Fairness metric.} A key question in the design of a scheduler is
what fairness metric should scheduling discipline target. Two
alternatives are resource and time-based fairness metrics. DRF and
similar schemes target resource fairness -- e.g., in DRF, contending
apps' dominant-resource shares are equalized. But, such
resource-centric approaches are a poor fit as argued above.

Time-based fairness is rooted in classic scheduling~\cite{drr}. In
this class of schemes, GPUs could each be allocated for a given amount
of time (``lease''). A recent variant~\cite{tiresias} attempts to
equalize ``attained service'', which is the total amount of GPU time
allocated to a job. When a lease expires, an available GPU is
allocated to a new app, where apps are considered for allocation in a
given order (e.g., round-robin~\cite{drr}, or least attained
service~\cite{tiresias}). Unfortunately, time-based approaches are not
resource-placement sensitive. It is difficult to encode placement
preferences into the attained service metric.


{\bf Efficiency.} Fairness-centered schemes may leave resources
fallow: GPUs available now may be a poor fit for the
farthest-from-fairshare app, but may be a good fit for another
app. Given the importance of efficient GPU utilization, our scheduling
discipline cannot afford to leave GPUs unused.


Overall, we need a new scheduling discipline that is not tied to short
task durations, is placement sensitive, does not rely on time- or
resource-based fairness, and puts efficiency on an equal footing with
fairness.



\subsection{Why a new scheduler architecture?}
ML apps that perform hyperparameter exploration use custom frameworks with internal
schedulers~\cite{hyperband, hyperdrive} to manage allocation of resources across the apps'
constituent jobs. The frameworks
typically classify jobs into multiple classes, such as ``good'',
``average'' or ``poor'', and the internal scheduler uses custom logic to
apportion resources among these classes.

One possible architecture for a scheduler is a
monolithic design that combines both cross-app and intra-app resource
allocation. Such a design is too complex and does not leave room for
apps' custom allocation logic for apportioning GPUs among many
internal ML job classes.

Thus, we consider instead a two-level scheduler architecture. The top
level scheduler is the app-specific one. The
bottom level manages allocation across apps.

Two state-of-the-art design approaches for the bottom-level
inter-app scheduler are {\em pessimistic} and {\em optimistic}.
Neither architecture is a good fit 
in our context.

A pessimistic architecture~\cite{mesos} means that available cluster
GPU resources are offered to {\em one} specific app at a time. 
To enforce placement preferences, the chosen ML app may reject an offer and
wait.  However the app may be forced to wait for many offers to get a
placement-optimal allocation, and such delays can become unbounded
due to ML tasks long durations, leading to sharing incentive
violation.

In optimistic architectures~\cite{omega}, {\em all} the resources in the
cluster are made visible and potentially available to all ML apps. Any
app can claim resources in a lock-free manner. The optimistic
architecture operates under the assumption that contention for the
same set of cluster resources across apps is unlikely, and even in the
case of a conflict, a simple machine-local conflict
resolution mechanism (e.g., scalar priority-based) can resolve
conflicts.  However, all ML apps typically compete for GPU resources,
and GPU clusters are heavily contended~\cite{philly_trace_analysis}. 
This can lead to many conflicts in an optimistic architecture. 
Also, if we rely excessively on a machine-local conflict resolution mechanism, 
we are not guaranteed convergence to a globally optimal solution that ensures
sharing incentive for all ML apps.

Thus, we need a two-level scheduler that is neither pessimistic nor
optimistic.  








































==> sections/policy_ignore.tex <==
\section{Finish-Time Fair Scheduler}


This section describes the finish-time fair policy  
and our implementation of that policy. 

First, is a description of the challenges in designing a scheduler 
for ML training workloads. These challenges are rooted in 
the attributes of ML apps. 
This leads to the description of the notion of finish-time fairness 
and the set of properties desired of a scheduler for ML apps. 
The four properties desired are sharing incentive, pareto-efficiency, 
envy freeness, and strategy proofness.

Next, is a description of the finish-time fair policy - 
a one-shot offline policy that achieves all these 
desired properties. 
However, the one-shot nature of this policy assumes perfect 
knowledge of ML app attributes. 

This leads to the description of the multi-shot 
finish-time fair policy that overcomes the 
assumption of perfect knowledge. It does not provably 
guarantee the sharing incentive property for all ML apps but 
maximizes the fraction of apps that get sharing incentive. 

\subsection{ML App Scheduling Challenges}

A scheduler for ML training workload is responsible for 
allocating GPUs to ML apps. 

The overall execution time \ie the finish-time of an ML app is 
primarily decided by the GPU allocation, which is represented as 
a vector - $\vec{G}$. 
$\vec{G}$ has dimensions equal to the number of GPUs that can be 
allocated and each element can be in the range $[0, 1]$. 

The amount of GPUs allocated - $||\vec{G}||_{1}$, limits 
the amount of parallelism 
that the ML app gets and hence the speedup in execution. 
ML apps execute one task per GPU and hence the task allocation vector 
is exactly the same as the GPU allocation vector ($\vec{G}$). 
Additionally, the execution time of an ML app is dependent on the 
{\em relative placement of its GPUs} and the {\em total work}.

\subsubsection{Relative Placement of tasks}
ML apps perform work in several iterations. 
Each iteration has computation followed by communication. 
Tasks compute updates to the model parameters followed 
by an aggregation of parameter updates every iteration~\cite{}.  

Ideally, the speedup in the finish-time of ML app should be 
linear in the number of tasks it can run 
\ie~the amount of GPUs that are allocated to the ML app ($||\vec{G}||_{1}$). 
However, compute resources sit idle during the communication phase 
and a less than linear speedup is observed.  
Different ML apps have different computation to 
communication ratios~\cite{}, have optimizations to overlap 
communication with computation to different degrees~\cite{}, 
and may have sparser updates as training progresses~\cite{}. 
All these factors determine the magnitude of the communication 
overheads incurred after tasks finish computation in an iteration. 
In such a scenario, the relative placement of tasks matters.
Sensitivity to relative placement of tasks is determined by 
the magnitude of these communication overheads. 
This is captured via a slowdown factor, denoted by 
$S(\vec{G})$ and is dependent on the task allocation 
vector ($\vec{G}$). 
Ideally, the speedup in the finish-time of ML app should be 
linear in the amount of tasks it can run ($||\vec{G}||_{1}$). 
$S(\vec{G})$ denotes the mulitiplicative factor by 
which an ML app is slowed down. 




\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{figures/rp-unaware-example.pdf} 
    \caption{Allocation with and without {\em relative placement awareness}}
    \label{fig:rp-unaware-example}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{figures/efficient-fair.pdf} 
    \caption{Relative Placement Aware Fair Allocation with and without Efficiency}
    \label{fig:efficient-fair}
\end{figure}

In essence, the finish-time ($F$) of an ML app 
is a function ($f$) of  
the amount of allocated GPUs ($||\vec{G}||_{1}$), 
the slowdown due to the relative placement of the 
allocated GPUs ($S(\vec{G})$) 
and the estimate of total work to be executed ($W$). 
\begin{equation} \label{eq:finish-time}
\begin{split}
    F &= f(\vec{G}, W) \\
      &= \frac{S(\vec{G})*W}{||\vec{G}||_{1}}
\end{split}
\end{equation}
This has implications on {\em what fairness means for ML apps} and 
{\em how to schedule ML apps in a fair and efficient manner}. 
The following examples explore these questions in further detail. 

\subsubsection{Examples}
Consider $N$ ML apps that need to be scheduled on $||\vec{R}||_{1}$ GPUs. 
$\vec{R}$ represents the total GPU resources to be allocated. 
The number of dimensions in $\vec{R}$ is the total number of GPUs and 
each element in $\vec{R}$ is $1$. 
Existing fair schedulers~\cite{drf, quincy, delay} 
that try to equalize the tasks allocated~\cite{quincy} or 
dominant share allocated~\cite{drf}, 
lead to an allocation of $\frac{||\vec{R}||_{1}}{N}$ GPUs to each app
~\footnote{Assume $||\vec{R}||_{1} > N$ for this hypothetical case and 
that each app has no upper limit on number of GPUs demanded.}. 
These fair schedulers typically assign an arbitrary set of 
$\frac{||\vec{R}||_{1}}{N}$ GPUs to each app with some of these schemes 
accounting for data-local task placement~\cite{delay, quincy}. 
This means that each app gets $\frac{||\vec{R}||_{1}}{N}$ 
GPUs with arbitrary relative placement. 
In the example in Figure~\ref{fig:rp-unaware-example},  
$4$ jobs are contending for $8$ GPUs spread 
across $2$ servers. All apps get $2$ GPUs, however 
app $A_{3}$ and app $A_{4}$ have GPUs spread across $2$ servers 
and get a relative placement 
worse-off than app $A_{1}$ and App $A_{2}$ that have GPUs consolidated 
on a single server. 
This makes existing schemes {\em relative placement unaware} - 
none of the existing schemes have ways to express and meet 
relative placement preferences for the allocated set of GPUs.  

A simple {\em relative placement aware} fair scheme would be to 
divide the $||\vec{R}||_{1}$ GPUs into $N$ congruent sets
\footnote{Two GPU sets are congruent if the cardinality and 
spatial placement of GPUs relative to each other in both of 
these sets is exactly the same. The notion of congruence can 
further be weakened for the case of ML Apps. Two sets are 
congruent if the slowest network interconnect between GPUs is the 
same for both the sets -- as the slowest interconnect dictates the 
network overheads in the case of synchronous SGD.} 
and assign each set to each ML app. 
Continuing the same $4$ apps example with $8$ GPUs and $2$ servers, 
such a relative placement aware fair allocation is shown in 
Figure~\ref{fig:rp-unaware-example}. 
This allocation is fair for ML apps because the relative placement of 
GPUs allocated to each app is exactly the same. 

However, not all ML apps have similar relative placement preferences 
as highlighted in Figure~\ref{fig:placement}. 
The job throughput for Inceptionv3 remains the same 
even when GPUs allocated are staggered across servers, 
whereas, with this staggered relative placement of GPUs 
the job throughput for VGG16 halves. 
This makes an app training Inceptionv3 model 
relative placement insensitive \ie 
the slowdown, $S(\vec{G})$, is \mytilde 1 
whereas an app training VGG16 is quite sensitive 
to relative placement of GPUs and has a slowdown, 
$S(\vec{G})$, of \mytilde 2. 

In practice, different apps have different relative placement 
preferences \ie~different slowdowns $S(\vec{G})$. 

For the example in Figure~\ref{fig:efficient-fair}, 
dividing the GPUs in $3$ servers across $2$ apps 
in congruent sets leads to a relative placement aware 
fair allocation. However, only app $A_{1}$ is relative placement 
sensitive while app $A_{2}$ is not, so an alternative 
allocation that is not congruent only improves the 
finish-time for app $A_{2}$ with no changes to the finish-time 
of app $A_{2}$. This still remains a relative placement aware 
fair allocation while improving efficiency.

This brings us to key goals in \name{} - 
\begin{enumerate}
    \item Define a new fairness metric that captures whether an 
    allocation is a {\em relative placement aware} fair allocation
    or not. This also means that such a metric should encompass 
    relative placement preferences that vary across ML apps.
    \item Design a GPU resource allocation mechanism for ML apps ($\vec{G}$) 
    that is fair, where fairness is measured in terms of the new fairness metric, 
    and at the same time maximizes efficiency.
\end{enumerate}

\subsection{Finish-Time Fairness}
\name{} proposes a new metric called as finish-time fairness, $\rho$. 
\begin{equation} \label{eq:finish-time-fairness}
    \begin{split}
        \rho &= F_{id}/F_{sh} \\
             &= \frac{F_{id}*||\vec{G}||_{1}}{S(\vec{G})*W}
    \end{split}
\end{equation}
Here, $F_{id}$ is the independent finish-time and 
$F_{sh}$ is the shared finish-time. 

The shared finish-time, $F_{sh}$, is the finish-time of the app 
in the shared cluster and is a function of the GPU allocation 
vector ($\vec{G}$). Specifically, it is dependent on 
the amount of GPUs allocated $||\vec{G}||_{1}$, 
the slowdown factor due to the allocation $S(\vec{G})$, 
and the total work $W$. 
Finish-time fairness, $\rho$, tracks {\em long-term} fairness. 
as it tracks the shared finish-time of the ML app. 
It is also {\em relative placement aware} due to 
the dependence of $\rho$ on $||\vec{G}||_{1}$ and $S(\vec{G})$. 

The independent finish-time, $F_{id}$, is the finish-time of the 
ML app in its own independent and exclusive $\frac{1}{N}$ share of 
the cluster.
Note that if the total resources in the cluster is $\vec{R}$, each 
ML App is allocated $\frac{||\vec{R}||_{1}}{N}$ GPUs. 
Each $\frac{||\vec{R}||_{1}}{N}$ set of GPUs is congruent. 
$F_{id}$ can be considered a constant and normalizes the values 
of $\rho$. 

\subsubsection{Desired Allocation Properties}
The ideal fair scheme desired is the one that allocates resources ($\vec{G}$) 
to each ML app such that the property $\rho \geq 1$ i.e. $F_{id} \geq F_{sh}$ 
is guaranteed to each ML app. 

Formally, the properties desired from a fair scheduler for ML apps are -
\begin{itemize}
    \item {\it Sharing Incentive} - {\bf SI}: $\rho \ge 1$. The finish-time of an app in the shared 
    cluster ($F_{sh}$) should be less than the finish-time of the app in its own independent
    and exclusive share of the cluster ($F_{id}$).
    \item {\it Pareto-Efficiency} - {\bf PE}: The finish-time of an app can only be decreased 
    at the expense of an increase in finish-time of some other app. 
    \item {\it Envy-Freeness} - {\bf EF}: No app should prefer the resource allocation 
    of some other app. 
    \item {\it Strategy-Proofness} - {\bf SP}: All apps should truthfully report all inputs 
    needed for allocating resources. 
\end{itemize}

\subsubsection{Examples}
To better understand the properties consider the 
example in Figure~\ref{fig:rp-unaware-example}. 
The allocation on the left does not provide any of 
{\bf SI}, {\bf PE} and {\bf EF}. 
{\bf SI} is violated as the independent finish-time, {\bf $F_{id}$}, 
for app $A_{3}$ and app $A_{4}$ with the congruent GPU allocations on 
the right in Figure~\ref{fig:rp-unaware-example} is 
less than the shared finish-time, {\bf $F_{sh}$} with the 
current allocations on the left. 
{\bf PE} is violated as app $A_{3}$ and app $A_{4}$ can exchange 
resources amongst themselves to yield the allocation on the right 
to improve their finish-time without adversely affecting any 
other apps finish-time. 
{\bf EF} is violated as app $A_{3}$ prefers the allocation of app $A_{2}$.

Consider another example shown in Figure~\ref{fig:efficient-fair}. 
The allocation on the left provides {\bf SI} and {\bf EF}, however 
{\bf PE} is violated. 
{\bf PE} is violated because the allocation on the right improves 
finish-time of app $A_{2}$ without any effect on the finish-time of app $A_{1}$. 

Nothing can be said about {\bf SP} without knowing the exact 
allocation mechanism in both the above examples.

\subsubsection{Existing Allocation Policies}
The desired allocation policy should guarantee all the above properties. 
Existing allocation policies focus on a different fairness metric and are 
instantaneously fair. 
The DRF~\cite{drf} allocation policy equalizes the dominant resource shares 
instantaneously at every scheduling decision, 
while Quincy~\cite{quincy} instantaneously equalizes the number of 
tasks allocated while also minimizing data movement costs. These data movement 
costs only capture input data locality for tasks. 
None of the above schemes take a long-term view of fairness as desired by 
finish-time fairness. 
Also, none of the above schemes are relative placement aware as is desired 
by tasks in ML apps. 
Carbyne~\cite{carbyne} takes a long-term view of fairness via altruisms, 
however does not encode relative placement awareness for tasks. 
\begin{theorem}
    Existing fair allocation policies - DRF, Quincy, and Carbyne - do not 
    guarantee finish-time fairness. 
\end{theorem}
\begin{proof}
    These policies do not guarantee {\bf SI} at the least. 
    All these policies can yield the relative placement unaware allocation in  
    Figure~\ref{fig:rp-unaware-example} which violates {\bf SI}.
\end{proof}

The allocation policy in \name{} improves on these existing policies and 
guarantees all the above properties.

\subsection{Offline Finish-time Fair Allocation Policy}
\floatname{algorithm}{Pseudocode}
\begin{algorithm}[t!]

\begin{scriptsize}
\begin{algorithmic}[1]

\State Applications \{$\textit{A}_i$\} \Comment{set of apps}
\State Bids $\mathbb{\rho}_i(.)$ \Comment{valuation function for each app $i$}
\State Resources $\myvec{R}$ \Comment{resource set available for auction}
\State OUTPUT: Resource Allocations $\myvec{G}_i$ \Comment{resource allocation for each app $i$}

\Statex

\Procedure{auction}{} 
    \State $\myvec{G}_{i,pf}$ = arg max $\prod_i \mathbb{\rho}_i(\myvec{G_{i}})$  \Comment{proportional fair (pf) allocation per app $i$}
    \State $\myvec{G}^{-i}_{j,pf}$ = arg max $\prod_{j != i} \mathbb{\rho}_j(\myvec{G_{j}})$  \Comment{pf allocation per app $j$ without app $i$}
    \State $c_i$ = $\frac{\prod_{j != i} \mathbb{\rho}_j(\myvec{G}_{j,pf})}{\prod_{j != i} \mathbb{\rho}_j(\myvec{G}^{-i}_{j,pf})}$
    \State $\myvec{G_i}$ = $c_i$ * $\myvec{G}_{i,pf}$ \Comment{allocation per app $i$} 
\EndProcedure

\State

\Procedure{multiShotAuction}{}
    \While{True}
    \If{$timeSinceLastAuction > lease$} 
    \State{$\myvec{G_i}$ = \textsc{auction}({$\mathbb{\rho'}_i(.)$})} \Comment{updated bids from apps}
    \EndIf
    \EndWhile
\EndProcedure

\State

\Procedure{onlineAuction}{}
    \State \textsc{onResourceAvailableEvent} $\vec{R}$:
    \State $A_{S}$ = \textsc{sort}(${A_i}$) on $\rho_{i}$
    \State $A_{f}$ = get top 1 - $f$ fraction of apps from $A_{S}$
    \State{$\myvec{G_i}$ = \textsc{auction}({$\mathbb{\rho'}_i(.)$})} \Comment{updated bids from apps in $A_{f}$}
\EndProcedure

\end{algorithmic}
\end{scriptsize}
\caption{Partial Allocation Mechanism}
\label{alg:pam}
\end{algorithm}

The finish-time fairness $\rho_{i}(.)$ for an ML app $A_{i}$ is a function  
of the GPU allocation $\vec{G_{i}}$ that it receives. 
The allocation policy takes these $\rho_{i}(.)$'s as inputs and 
outputs allocations $\vec{G_{i}}$. 

In \name{}, one of the main contribution is that the allocation policy 
is mapped to an {\em auction}. 
It treats the available GPUs as arbitrarily divisible goods to be 
auctioned to all the ML apps with $\rho_{i}(.)$'s as bids submitted by ML apps. 

Auctions are described next. 

\subsubsection{Auction}
Details of the inputs necessary to run the auction are given first, 
followed by how the auction works given these inputs. 

{\noindent \bf Inputs: Resources and Bids.} $\vec{R}$ represents 
the total GPU resources to be auctioned. 
Each element in $\vec{R}$ is $1$ and the number of dimensions in $\vec{R}$ 
is the number of GPUs to be auctioned.  

Each ML app bids for these resources. 
The bid for each ML app consists of the estimated 
finish-time fair metric ($\rho_{i}$) values for several 
different GPU allocations ($\vec{G}_{i}$). 
Each element in $\vec{G}_{i}$ can be a fraction in the range $[0, 1]$.  
These fractions can be realized in practice by time-multiplexing the usage of GPUs. 
For example, an allocation of $0.1$ would mean that $10\%$ of time on that GPU is 
reserved for that app. 

{\noindent \bf Auction Overview. } The partial allocation (PA) mechanism~\cite{nopaymentfair} 
is used to pick the winning resource allocations per app. 
Pseudocode~\ref{alg:pam}, line $5$ shows the PA mechanism.

PA starts with an initial proportional fair allocation that guarantees all the above 
properties except {\bf SP}. It enforces truth-telling \ie~{\bf SP} via the notion 
of hidden payments. There are two aspects to auctions that are described next. 

{\noindent \bf 1. Initial allocation.} PA starts by calculating an 
intrinsically proportional fair allocation $\vec{G_{i, pf}}$ for each app $A_{i}$ 
by maximizing the product of the valuation functions \ie~the finish-time fair metric values
for all apps (Pseudocode~\ref{alg:pam}, line $6$). 
This allocation satisfies all the properties except {\bf SP}. 

{\noindent \bf 2. Incentivizing Truth Telling.} To induce truthful reporting of the bids, 
the PA mechanism allocates app $A_{i}$ only a fraction $c_{i} < 1$ of $A_{i}$'s proportional 
fair allocation $\vec{G_{i, pf}}$, and takes $1 - c_{i}$ as a hidden payment 
(Pseudocode~\ref{alg:pam}, line $9$). The $c_i$ is directly proportional to the 
decrease in collective valution of the other bidding apps in a market with and without 
app $A_{i}$ (Pseudocode~\ref{alg:pam}, line $8$). This yields the final allocation 
$\vec{G_{i}}$ for app $A_{i}$ (Pseudocode~\ref{alg:pam}, line $9$).

Note that, $\vec{G_{i}}$ is not a market-clearing allocation and there could be 
unallocated GPUs left over unallocated due to hidden payments. 
As a result, PA is not work-conserving. 

\begin{theorem}
    Auction in \name{} guarantees {\bf SI}, {\bf PE}, {\bf EF}, and {\bf SP}.
\end{theorem}
\begin{proof}
    Refer to Appendix.
\end{proof}

We make an assumption here that the valuation function $\rho_{i}(.)$ 
and indirectly the total work $W_{i}$ as well as the slowdown factor 
function $S_{i}(.)$ for each app $A_{i}$ do not change with time and 
are accurately known. 
In practice, the total work $W_{i}$ as well as the slowdown factor 
function $S_{i}(.)$ change with time and thus the estimate of 
$\rho_{i}(.)$ changes with time. 

\subsubsection{Multi-shot Auctions}
To overcome the above assumption, we introduce 
the notion of {\em Multi-shot Auctions} (line $12$ -- $18$ in 
Pseudocode~\ref{alg:pam}). 

With multi-shot auctions, the outcome of allocations from an 
auction are binding only for a {\em lease} duration. 
At the end of this lease, each app submits its updated bid -- 
the valuation function $\rho'_{i}(.)$. 
There is a slight change in the way apps are expected to 
report these updated bids.  
These $\rho'_{i}$ estimates are provided on the remaining work. 
$F_{sh}$ is the shared finish-time for completing the remaining work 
and not the total work. This is important for provability of 
strategy proofness and incentivizing truth-telling of $\rho'_{i}$ values. 
The auction is then conducted again with these 
updated bids to get the updated 
resource allocations $G_{i}$ for all apps.

\begin{theorem}
    Multi-shot Auctions in \name{} guarantee {\bf PE}, {\bf EF}, and {\bf SP}.
\end{theorem}
\begin{proof}
    Refer to Appendix.
\end{proof}

Multi-shot auctions do not provably guarantee 
sharing incentive {\bf SI}. 
Consider the case when the number of apps far 
exceeds the total number of GPUs in the cluster. 
In such a case, it is possible 
that a certain app repeatedly gets 
no allocation across auctions and is starved.  
This is so because the auctions take $\rho'_{i}(.)$ 
valuation functions as input and do not account 
for the effect of starvation time for the app. 

Also, the allocation policy so far does not account for 
online arrivals of apps. 

\subsubsection{Online Auctions}
To handle the online case and to maximize the 
number of apps that are guaranteed sharing incentive {\bf SI}, 
we propose the online auction scheme in 
Pseudocode~\ref{alg:pam}, line $20$. 

To handle the online case, auctions are triggered 
on any resource available event. 

To maximize the number of apps that are guaranteed 
sharing incentive we limit the visibility of apps that 
are included in the auction. 
The resources are auctioned to the first $1 - f$ fraction of ML apps 
sorted in decreasing order of $\rho$ values. 
Higher $f$ leads to stronger guarantees on finish-time fairness. 
Lower $f$, which trade-off fairness, allows more apps in the auction 
and increases the likelihood to find relative placement efficient allocations 
for the available set of GPUs among the apps in the auction. 









==> sections/policy_old.tex <==
\section{Finish-Time Fair Policy}
\label{sec:policy}






To achieve sharing incentive on the finish-time fairness metric
$\rho$, we propose a {\em max-min} fair allocation policy. This leads
us to an allocation that corresponds to the solution of the following
optimization program:

\begin{alignat*}{2}
    \text{min } &\epsilon_{max} &\tag{2} \\
    \text{subject to} \\
    \epsilon_i &\le \epsilon_{max} &\forall \text{ app } i \in 1 \text{to} N \tag{3} \\
    \rho_i &\le N + \epsilon_i &\forall \text{ app } i \in 1 \text{to} N \tag{4}\\
    \sum_{i} \mathcal{G}_{x,y,i} &= 1 &\forall \text{ gpu } x \text{ on machine } y \tag{5}\\
    \rho_i &= \mathcal{F}_{i}(\myvec{[\mathcal{G}_{x,y,i}]_{x,y}}, \myvec{\mathcal{W}_{i}}, \mathcal{S}_{i}) &\forall \text{ app } i \tag{6}\\
    \mathcal{G}_{x,y,i} &\in \{0, 1\} &\forall x, y, i \tag{7}
\end{alignat*}



In the above optimization formulation, given $N$, apps we minimize the
maximum deviation $\epsilon_{max}$ from $N$, which is the ideal value
of $\rho$.  $\myvec{[\mathcal{G}_{x,y,i}]_{x,y}}$ is the GPU
allocation vector for an ML app $i$, where $\mathcal{G}_{x,y,i}$ is
set if GPU $x$ on machine $y$ is allocated to an app $i$.  The GPU
resource allocation vector encodes the amount, the type and the
placement of GPUs allocated to an app.  $\myvec{\mathcal{W}_i}$ is the estimate of total work
for an app $i$.  The finish-time fairness metric ($\rho$) is typically
a function, $\mathcal{F}_{i}$, of the resource allocation
($\myvec{[\mathcal{G}_{x,y,i}]_{x,y}}$) and the estimate of total work
for all the constituent jobs ($\myvec{\mathcal{W}_i}$).
$\mathcal{F}_i$ captures the placement sensitivity, $\mathcal{S}_{i}$,
of the running time for app $i$. Because of this property of
$\mathcal{F}_{i}$, the above formulation accounts for cluster
efficiency in addition to fairness.

We first show that the solution to the above induces sharing
incentive in the case where all apps start at the same time, and
resources are apportioned \emph{offline} prior to apps starting.




\vspace{0.05in}
\noindent  
{\bf Observation:}
The above solution enforces sharing incentive.
\vspace{0.05in}

\noindent
{\bf Justification:} Say there are $N$ ML apps.  Divide the
cluster into $N$ ideal shares: each corresponding to a dedicated $1/N$
cluster.  By definition, this allocation with dedicated resources
offers sharing incentive\footnote{this assumes linear scaling in app
  running time when the app runs in $1/N$ dedicated cluster}, \ie
$\rho_i = N$, $\forall i$, which implies $\epsilon_{max} = 0$.  Given
this, the optimal solution to the above program is one with
$\epsilon_{max} \le 0$, which implies $\rho_i \le N$, $\forall i$.
Thus, the optimal solution offers sharing incentive.

\vspace{0.05in}






In practice, we cannot assume all apps start at the same time. Also,
the finish time metric is time-varying. %
ML apps placement sensitivity
($\mathcal{S}_{i}$) is often not known accurately ahead of time, and
becomes apparent only as jobs execute.  Also, estimated total work
($\myvec{\mathcal{W}_i}$) depends on convergence properties of the
training algorithm and keeps changing with time - with the magnitude
of changes diminishing over time. It also depends on how many
constituent jobs the app's internal scheduler decides to keep alive or
terminate; $\myvec{\mathcal{W}_i}$ changes substantially when the app
terminates a job that is exploring ``poor'' hyperparameter settings.





\noindent
{\bf A Strawman.} To address this, one could consider a practical
``online'' strawman wherein each resource allocation decision is
binding for a ``lease'' duration after which the resource is up for
reallocation.
Each app can send updated values of $\rho$ to the \arbiter{} just
before a reallocation.  The \arbiter{} can then use these updated
values to reallocate resources to the app with the {\em worst} $\rho$.
However, there are two issues in this strawman.

First, allocating to just one app  can be inefficient.  The
\arbiter{} may end up allocating GPUs to the app in a placement
insensitive manner.  The new allocation may span across many machines
or racks relative to the app's currently held GPUs, and can lead
to inefficient overall GPU use.
Given the long-term focus of our fairness metric, this makes the case
for relaxing strict tracking of finish-time fairness and increasing
the {\em visibility} of available resources, because offering resource
to a different app that places better on the available GPUs can be
more {\em efficient}.

Second, the \arbiter{} trusts the apps' to be truthful about their
finish-time fair metric.  At each reallocation event, an adversarial
app can obtain many of the available GPUs by over-reporting the value
of $\rho$, which can hurt honest apps' sharing incentives.  This makes
the case for incentivizing apps' {\em truthfulness} in reporting their
finish-time fair metric.







==> sections/semioptimistic.tex <==
\section{Semi-Optimistic Scheduler}
\label{sec:semiopt}

\floatname{algorithm}{Pseudocode}
\begin{algorithm}[t!]

\begin{scriptsize}
\begin{algorithmic}[1]

\State Applications \{$\textit{A}_i$\} \Comment{set of active apps}
\State Bids $\mathbb{B}$

\Statex

\Procedure{offerResources}{$\myvec{R}$} \Comment{triggered when resources $\myvec{R}$ are available}
    \State $\mathbb{A}_s$ = \textsc{sort}($\mathbb{A}_f$) on \textsc{metric}($\textit{A}_i$) \Comment{default \textsc{metric} is $\rho$}
    \State $\mathbb{A}_f$ = get top $1-f$ fraction of apps from $\mathbb{A}_s$ \Comment{$f$ is fairness knob}
    \State auction resources $\myvec{R}$ to all apps in $\mathbb{A}_f$
    \State $\mathbb{B}$ = []
    \ForAll{$\textit{A}_i \in \mathbb{A}_f$}
        \State \textsc{auction}($\myvec{R}$) to $\textit{A}_i$ \Comment{send an offer to \agent{}}
        \State $\textit{B}_i$ = $\textit{A}_i$.\textsc{prepareBids}($\myvec{R}$) \Comment{get bid table $\textit{B}_i$ = \{ ($\myvec{R}_{s}$, $\rho_{i,s}$) \} from \agent{} for different subsets $\myvec{R}_{s} \subset \myvec{R}$}
		\State $\mathbb{B}$.\textsc{append}($\textit{B}_i$)
	\EndFor
    \State $\mathbb{B}_{w}$ = \textsc{partialAllocation}($\mathbb{B}$)
    \ForAll{($\textit{A}_{ij}$, $\myvec{R}_{ij}$, $\rho_{ij}$) $\in$ $\mathbb{B}_w$}
        \State assign resources $\myvec{R}_{ij}$ to job $\textit{J}_j$ in app $\textit{A}_i$ for $lease$ duration
        \State $\rho_i$ = \textsc{max}($\rho_i$, $\rho_{ij}$)
    \EndFor
\EndProcedure

\end{algorithmic}
\end{scriptsize}
\caption{\name{} \arbiter{}}
\label{alg:tgs}
\end{algorithm}

In \name{}, we separate {\em visibility} from {\em allocation} using a
semi-optimistic online scheduler at the \arbiter{}. The design helps
us control both efficiency and fairness.





The \arbiter{} implements a generalized version of the online
algorithm presented before (Pseudocode~\ref{alg:tgs}) with
modifications to improve efficiency and incentivize truth
telling. After first asking all apps to report their current $\rho$,
the \arbiter{} makes any available GPU resource visible to $1-f$
fraction of ML apps sorted in decreasing order of $\rho$s reported.
Higher $f$ leads to stronger guarantees on finish-time fairness. Lower
$f$, which trade-off fairness, allows the \arbiter{} to find placement
efficient allocations.  We evaluate the sensitivity of of \name{} to values of $f$ in
Section~\ref{sec:eval}.

The \arbiter{} computes a globally-optimal and conflict-avoiding
allocation of GPUs. It does so by treating available GPUs as (bundled)
goods to be auctioned to the $1-f$ apps. Multiple apps can bid for
overlapping sets of GPUs. The auction allocates each GPU to exactly
one app, thus avoiding any form of conflict resolution or concurrency
control~\cite{omega}. The set of app-GPU pairs are selected to
optimize a ``social objective'': instead of uniformly spreading GPUs
across the bidding apps, the \arbiter{} preferentially allocates
to apps that pack well and collectively see the greatest aggregate
improvement in their finish-time  metrics.

We describe our auctions next. Truth-telling is supported by design.









\subsection{Auctions}
\label{auction}







We first describe the inputs necessary to run the auction, then how
the auction works given these inputs, and finally the fairness and
efficiency it achieves. We defer discussion of how to gather inputs to Section~\ref{interfaces}.

\noindent
{\bf Inputs: Resource offer, and bids.}  Let $\myvec{R}$ be the set of
available GPUs that are offered to the $1-f$ fraction of far-from-fair
(worst $\rho$) apps.
Each dimension in $\myvec{R}$ represents the number of unused GPUs in
a given machine in the cluster.

Each app on receiving an offer for
$\myvec{R}$ replies with a single {\em bid}.  Every ML app tries to
win fractions of each of the machines' unused GPUs.  In a machine with
$n$ available GPUs, the permissible fractions are $\frac{1}{n}$,
$\frac{2}{n}$, \dots, $1$.

 

App $i$'s bid is a {\em valuation function}, $\mathcal{V}_i$, that
maps different allocations, $\myvec{R}_a$, to app $i$'s new
finish-time metric, $\rho_{i,a}$, that results from adding the
$\myvec{R}_a$ GPUs to the existing GPUs that app $i$ currently has,
and assuming that all GPUs (existing and newly added) are used from
this point on till app $i$'s completion. Each allocation $\myvec{R}_a$
identifies the fraction of each machine's free GPU resources desired
by the app.

Given discrete subsets of resources, $\mathcal{V}_i$ for app $i$ is a
table, with a row for different choices for $\myvec{R}_a$. One of the
rows covers the case where the apps receives no new allocation
($\myvec{R}_a$ is all zeros) with the corresponding valuation being
the app's current finish-time fairness metric. 



\noindent
{\bf Auction overview.}  Once all the bids are received by the
\arbiter{}, it applies a {\em partial allocation (PA)}
mechanism~\cite{nopaymentfair} to pick the winning resource
allocations per app. Some auction-participating apps may receive no
new allocations.  Pseudocode~\ref{alg:pam} shows the PA mechanism.

PA starts with an initial proportional fair allocation, then it
enforces truth-telling. It may leave GPUs unallocated, which we then
assign in a work conserving manner. We describe these three aspects of
the auction next. Then, we describe how our auction trades off
fairness and efficiency in the short term, but ensures finish time
fairness in the long term.


\noindent
{\bf 1. Initial allocation.}  PA starts by calculating an intrinsically
{\em proportionally fair} allocation $\myvec{R}_{i,pf}$ for each app
$i$ (line 6) by maximizing the product of valuation functions
$\mathcal{V}$. The resulting solution is also {\em Pareto-efficient}:
no app's valuation can be improved without hurting some other app's
valuation.

\noindent\textbf{2. Incentivizing Truth Telling.}  To induce truthful
reporting of the valuation functions $\mathcal{V}_i$, the PA mechanism
allocates app $i$ only a fraction $c_i<1$ of $i$'s proportional fair
allocation $\myvec{R}_{i,pf}$, and takes the fraction $1-c_i$ as a
{\em hidden payment} (Pseudocode~\ref{alg:pam}). The $c_i$
is directly proportional to the decrease in collective valuation of
the other bidding apps in a market with and without app $i$ (lines 7 and 8).
This yields the final allocation $\myvec{R_i}$ for app $i$ (line 9).

In~\cite{nopaymentfair}, it is shown that this mechanism incentivizes
{\em truth-telling} of the valuation function, $\mathcal{V}$, under
the assumption that $\mathcal{V}$ is homogeneous with degree one
\ie~$\mathcal{V}(k*\myvec{R_a}) = k*\mathcal{V}(\myvec{R_a})$.  This
assumption holds true in our setting as well: %
when we increase an app's allocation from $\myvec{R_a}$ to $k*\myvec{R_a}$,
the relative placement of allocated machines in $\myvec{R_a}$ and
$k*\myvec{R_a}$ does not change (because we allocate more GPUs on the
same set of machines) and the value of $\rho$, which is the app's
valuation function, improves $k$ times \ie~$\rho_{improved} =
\frac{\rho}{k}$. %

\noindent\textbf{3. Leftover Allocation.} Note that, $\myvec{R_i}$ is
not a market-clearing allocation and there could be GPUs left over
unallocated due to hidden payments.  The PA mechanism guarantees that
at most $\frac{1}{e}$ worst-case fraction of total available resources are
leftover (in practice we find this to be much lower). At the end of PA mechanism, our \arbiter{}
allocates all leftover GPUs to apps {\em not} participating in the
auction in a placement-sensitive manner.  Leftover allocation is made
one GPU at a time to these apps in a way that the new GPU is placed on
one of the machines that is already a part of an existing allocation
for that app. When many such candidate apps exist for a GPU, one of
the apps is picked at random. This ensures that \name{} allocates all
available GPUs and is {\em work conserving}.

From the perspective of an app, say $k$, that did not participate in
the auction, the set of leftover GPUs is essentially random.
In particular, there is no way
for $k$ to be strategic to win allocation of leftover GPUs during an
auction. Thus, we preserve the overall truthfulness and Pareto
efficiency properties of our cluster scheduler.

\noindent\textbf{Short-term efficiency, long-term fairness.} We now
return to how, via auctions, we are able to trade-off fairness on the
short-term, but the scheduler is still able to achieve fairness in the
long term. Consider a far-from-fair app $i$ that lost an auction. It
will appear in future auctions with much greater likelihood relative
to another less far-from-fair app $k$ that won the auction. This is
because, the winning app $k$ was allocated resources; as a result, it
will see its fairness metric improve; thus, it will eventually not
appear in the fraction $1-f$ of not-so-fairly-treated apps that
participate in future auctions. In contrast, $i$'s fairness metric
stays the same, and thus it will continue to appear in future
auctions. Further an app that loses multiple auctions will eventually
lose its lease on all resources and make no further progress, causing
its finish time metric to become unbounded. The next auction the
app participates in will likely see the app's bid winning, because
any non-zero GPU allocation to that app will lead to a huge
improvement in the app's valuation.





\subsection{Interfaces between \agent{} and ML App Scheduler}
\label{interfaces}

As mentioned in Section~\ref{sec:design}, an \agent{} co-resident with
an app helps the app participate in auctions. We now describe how 
\agent{}s prepare bids based on inputs provided by apps, the API
between an \agent{} and its app, and how \agent{}s integrate with
current hyper-parameter optimization schedulers.



{\noindent \textbf{Calculating $\boldsymbol{\rho}$.}} The \arbiter{}
probes all apps' \agent{}s prior to auctions for their current
finish-time fair metrics. In addition, if an app is chosen to
participate in an auction, its \agent{} needs to provide, as part of
its valuation function, estimates of the new $\rho$ resulting from
potential new resource allocations from the \arbiter{}. We now
describe how the \agent{} computes these estimates. For simplicity, we
focus on how the agent computes the new $\rho$ resulting from a
possible new allocation; calculating and reporting current $\rho$ upon
being probed by the \arbiter{} is similar. 


To calculate $\rho_{i,a}$ resulting from
being allocated a particular subset of GPUs $\myvec{R_a}$ in app $i$'s
valuation function table, the \agent{} follows these steps:

\begin{enumerate}
   \item Calculate the aggregate ($\myvec{G_{i,a}}$) of the GPU allocation
     vector in the bid ($\myvec{R_a}$) and the already assigned GPU
     allocation vector for app $i$: $\myvec{G_{i,a}}$ = $\myvec{R_a} +
     \myvec{[\mathcal{G}_{x,y,i}]_{x,y}}$.

   \item Obtain estimates of the app $i$'s total work, and total work
     left for each constituent job $j$ in $i$, i.e.,
     $\myvec{\mathcal{W}_{i,j}}$ and $\myvec{\mathcal{W'}_{i,j}}$,
     respectively (more on estimating these quantities this shortly).
     Work is measured in GPU-hours.
     
   \item Obtain the placement sensitivity for each job $j$ in app $i$,
     $\mathcal{S}_{i,j}$. We model $\mathcal{S}_{i,j}$ as the slowdown
     observed when GPUs allocated for the job span different
     networking boundaries. We explain this below. $\mathcal{S}_{i,j}
     \rightarrow 1$ indicates close-to-ideal placement.

     With an ideal placement, the running time of a job linearly
     scales with the number of GPUs ($\mathcal{G}$) \ie~$time =
     \frac{serialTime}{\mathcal{G}}$, where $serialTime$ is serial
     running time with a single GPU.  However, scaling is less than
     linear in proportion to the factor $\mathcal{S}_{i,j}$ depending
     on the topological spread of GPUs \ie~$time =
     \frac{serialTime}{\mathcal{G}*\mathcal{S}_{i,j}(\myvec{G})}$,
     where $\mathcal{S}_{i,j}(\myvec{G}) \le 1$ depends on the spread of
     GPUs in the GPU allocation vector $\myvec{G}$ of the job.  We
     typically have three values for $\mathcal{S}_{i,j}$, one each
     reflecting the case where GPUs span different slots in a machine;
     span multiple machines in a rack; and span
     racks. $\mathcal{S}_{i,j}$ also depends on the overhead of
     communication during training and includes the model parameter
     sizes, typical parameter gradient sizes, and any training time
     communication optimizations (more on estimating
     $\mathcal{S}_{i,j}$ shortly). 
     
   \item The \agent{} estimates the shared
     running time for app $i$ as:  $T_{SH,a} = min_j$ ($timeElapsed$
     + $\frac{ \mathcal{W'}_{i,j} }{ \myvec{G_{i,j,a}} *
       \mathcal{S}_{i}(\myvec{G_{i,j,a}}) }$), where
     $\myvec{G_{i,j,a}}$ is the allocation reserved for job $j$ in app
     $i$.  The $min$ in the calculation above reflects the fact that
     the job with the {\em best} hyper-parameters, i.e., the one that
     trains to a target accuracy fastest, is the one that determines
     the app's finish time. Note that given the overall app-level
     allocation $\myvec{G_{i,a}}$, the \agent{} computes the job-level
     $\myvec{G_{i,j,a}}$ allocation in a greedy manner, where GPUs are
     assigned to jobs in a placement sensitive manner.
     
   \item The \agent{} calculates the ideal running time as: \\ $T_{ID} =
     min_j$ ($\frac{ \mathcal{W}_{i,j} }{ \myvec{G_{ideal,i,j}} }$),
     where $\myvec{G_{ideal,i,j}}$ is the ideal GPU allocation
     vector. (Again, $min$ plays the same role as above.)  Each job
     has an upper limit on the number of tasks it can parallelize
     across; the ideal GPU allocation vector is thus the one with this
     maximum parallelism and best placement sensitivity.

   \item The \agent{} computes the estimate of finish-time
     fair metric for the app $i$ as: $\rho_{i,a} = \frac{T_{SH,a}}{T_{ID}}$.

   \item The \agent{} inserts $\myvec{R_a}$, $\rho_{i,a}$ in the
     valuation function table that it provides to the \arbiter{}.
\end{enumerate}




{\noindent \bf ML App Scheduler to Agent API.}  Note that preparation
of the bid requires the app-scheduler to provide the amount of total
work and work left per job in the app ($\myvec{\mathcal{W}_{i,j}}$ and
$\myvec{\mathcal{W'}_{i,j}}$), the placement sensitivity ($\mathcal{S}_{i,j}$),
and the maximum parallelism assigned per job
($\myvec{G_{ideal,i,j}}$).  Note that this is not static information,
as the placement sensitivity ($\mathcal{S}_{i,j}$) is dependent on the model and
the cluster environment (network technology and average interfering
traffic).  Also, the work left per-job depends on the convergence
properties of the job.  Thus, at the beginning of a bid preparation,
the \agent{} {\em pulls} this information from the ML app scheduler.

{\noindent \bf Obtaining Estimates from App Schedulers.} We now
discuss how existing app schedulers can be easily modified to provide
\agent{}s with the above needed information such that \agent{}s can
calculate their bids. We focus on HyperBand~\cite{hyperband} and
HyperDrive~\cite{hyperdrive}, two popular ML app schedulers for
hyperparameter optimization in model training.

{\em App scheduler background:} HyperBand launches several ML training
jobs each with user-configured equal ``priority'' \ie~equal
$\myvec{G_{ideal,i,j}}$ or equal maximum parallelism.  HyperBand kills
the bottom-half of jobs with poor convergence periodically after a
fixed number of iterations until a single job remains.

HyperDrive launches several ML training jobs with user-configured
equal priority \ie~equal maximum parallelism to begin with.  It
continually monitors the jobs' loss convergence properties to classify
jobs as {\em good}, {\em promising}, and {\em poor}. HyperDrive then
gives varying execution priorities to different jobs by controlling
the maximum parallelism $\myvec{G_{ideal,i,j}}$ for each constituent
job, with higher priorities for {\em good} jobs and terminating a job
as soon as it is classified as {\em poor}.

{\em Work estimation:} In either case, deciding which jobs to kill/keep, or into which
category to classify a job, is done by curve-fitting and estimating
the number of iterations to completion of the job. Jobs with too many
projected iterations to complete are killed (HyperBand) or classified
as poor (HyperDrive).  Thus, we minimally modify these schedulers to
report their internally-tracked projected iterations to completion for
each job as their estimates for the amount of work left.





{\em Placement sensitivity:} The only information that is typically
missing from app schedulers is the placement sensitivity
($\mathcal{S}_{i,j}$).  This requires profiling the iteration times
for different placement options for an app's jobs.  Luckily, we find
that all jobs within an app (especially those that share a model
structure, but differ in other hyper-parameters) typically have
correlated placement sensitivity. This helps with two practical
simplifications: First, we can use a single $\mathcal{S}_{i}$ for an
entire app $i$. Second, we can be opportunistic and exploit the
diversity in placement across constituent jobs in the app during their
initial few training iterations to measure the effect of different
placements in the cluster. Thus, over a small period of time, we can
get accurate measures of $\mathcal{S}_i$.




 







This concludes our discussion of how the \arbiter{} and \agent{} are designed and we next discuss how
these mechanisms are implemented in \name{}. 


